Airbert: In-domain Pretraining for Vision-and-Language Navigation

Vision-and-language navigation (VLN) aims to enable embodied agents to navigate in realistic environments using natural language instructions. Given the scarcity of domain-specific training data and the high diversity of image and language inputs, the generalization of VLN agents to unseen environments remains challenging. Recent methods explore pretraining to improve generalization, however, the use of generic image-caption datasets or existing small-scale VLN environments is suboptimal and results in limited improvements. In this work, we introduce BnB, a large-scale and diverse in-domain VLN dataset. We first collect image-caption (IC) pairs from hundreds of thousands of listings from online rental marketplaces. Using IC pairs we next propose automatic strategies to generate millions of VLN path-instruction (PI) pairs. We further propose a shuffling loss that improves the learning of temporal order inside PI pairs. We use BnB pretrain our Airbert model that can be adapted to discriminative and generative settings and show that it outperforms state of the art for Room-to-Room (R2R) navigation and Remote Referring Expression (REVERIE) benchmarks. Moreover, our in-domain pretraining significantly increases performance on a challenging few-shot VLN evaluation, where we train the model only on VLN instructions from a few houses.

==> sections/5.downstream.tex <==
\section{Applying \airbert~to VLN tasks}
\label{sec:downstream}
Our \airbert~can be readily integrated in both discriminative and generative models for different VLN tasks.
% We briefly describe how it is adapted in the R2R navigation~\cite{anderson2018r2r} and REVERIE remote referring expression~\cite{qi2020reverie} tasks.
% (i) R2R~\cite{anderson2018r2r}: navigation by following instructions; and
% (ii) REVERIE~\cite{qi2020reverie}: navigation and object localization through remove referring expressions.


\p{Discriminative Model: Navigation as Path-Selection}
features a set of human-annotated instructions describing trajectories in Matterport3D~\cite{Matterport3D} environments.
In the \emph{discriminative} setting, the navigation problem is formulated as a path selection task \cite{majumdar2020vlnbert}, where candidate paths are generated via beam search from a navigation agent such as \cite{tan2019envdrop} and the goal is to choose the best path among them.
We follow the setups as in \cite{majumdar2020vlnbert}.
The \airbert~is finetuned on R2R dataset in two stages: the first involves using \emph{masking} and \emph{shuffling} losses in a manner similar to \airbnb~PI pairs; in the second phase, we choose a positive candidate as one that arrives within 3m of the goal, and train a ranking model that contrasts against negative candidate paths.
% We compare multiple strategies to mine additional negative pairs (other than 3 negative candidates), and empirically show that negatives created using shuffling in fact outperform multiple other options.



\p{Generative Model: Recurrent VLN-BERT}
% \label{sec:downstream:reverie}
% \cite{qi2020reverie} requires an agent to find a remote object in a home based on an instruction that contains high-level navigation guidance and a specific object grounding expression. 
% The agent is expected to navigate to a viewpoint which contains the target object, and then identify it from a list of given objects.
% The \airbert~model is used as the backbone \emph{Recurrent VLN-BERT}~\cite{hong2021recurrentvln} in a similar way as in R2R navigation task, except that the objects are also concatenated in the visual transformer and the stop action is decided when an object token receives maximum attention score from the \cls~state token.
We plug \airbert~as the backbone of \emph{Recurrent VLN-BERT}~\cite{hong2021recurrentvln} for sequential action prediction.
Specifically, the language transformer first encodes the instruction via self-attention.
Then the embedded \cls~token in the instruction is used to track history and concatenated with observable navigable views in each action step.
Both self- and cross-attention on embedded instructions are employed to update the state and visual inputs.
The navigation view is selected by the attention scores from the state to vision tokens for each step.
Please refer to the appendix for additional model and implementation details.


==> tables/where.tex <==
%!TEX root = ../main.tex
\begin{table}[t]
\centering
\tabcolsep=0.10cm
\begin{tabular}{l cccc | c | cc}
\toprule
% \multicolumn{4}{c|}{\textbf{Pre-training}} & FT & \multicolumn{2}{c}{Success Rate} \\
% & CC & \airbnb-IC &  R2R & \airbnb-PI & R2R & \multicolumn{2}{c}{SR on Val} \\
& CC & R2R & \airbnb & R2R & \multicolumn{2}{c}{SR on Val} \\
& M+P & M & M+S & Rank & Seen & Unseen \\
\midrule
% \ding{172}--\ding{181} % seriffed fonts
% \ding{192}--\ding{201} % sans-seriffed fonts
% vanilla
% 1 & \ding{172} & - & \ding{173} & - & \ding{174}
1 & \checkmark &  \checkmark & - & \checkmark
    & 70.20 & 59.26 \\
% Replace CC  bnbMN_r2rM_r2rR_scratch
2 & - & \checkmark & \checkmark & \checkmark
    & 74.02 & 60.54 \\
% After CC imag-caption  bnbMN_r2rM_r2rR
% 3 & \ding{172} & \ding{173} & \ding{174} & - & \ding{175}
%     & 71.21 & 62.45 \\
% After CC imag-caption  bnbMS_r2rM_r2rR
% \ding{172} & -  & \ding{174}& \ding{173} & \ding{175}
%     & 74.34 & 63.69 \\
%    & 10.39 & 3.58 & 0.71 & 80.41 & 74.34
%    & 9.78 & 3.88 & 0.69 & 73.13 & 63.69 \\
% After R2R  r2rM_bnbMS_r2rR
% 4 & \ding{172} & - & \ding{173}& \ding{174}  & \ding{175}
%     & 73.84 & 62.71 \\
% After R2R  r2rM_bnbMS_r2rR - with best table 2 (same as 3.3)
3 & \checkmark & \checkmark & \checkmark & \checkmark
    & 73.57 & 66.52 \\
% After R2R  r2rM_bnbMS_r2rRS_indoor
% 1 & - & 3 & 2 & 4 & 71.69 & 63.47 \\
% bnbMN_bnbMS_r2rM_r2rRS
% 6 & \ding{172} & \ding{173} & \ding{175}& \ding{174}  & \ding{176}
%      & 75.59 & 65.52 \\
% 7 & \ding{172} & \ding{173} & \ding{175}& \ding{174}*  & \ding{176}
%      & 78? & 70? \\
% % bnbMN_r2rM_bnbMS_r2rRS
% \ding{172} & \ding{173} & \ding{174} & \ding{175} & \ding{176}
%     & xx.xx & xx.xx \\

\bottomrule
\end{tabular}
\vspace{-2mm}
\caption{
Performance comparison between various stage-wise pre-training methods (first 4 columns), followed by fine-tuning on R2R with the ranking loss.
The number inside the circle indicates the stage.
\textbf{Dataset} acronyms on first row:
CC: image-caption pairs from Conceptual Captions;
\airbnb-IC: image-caption pairs from \airbnb;
\airbnb-PI: trajectory-instruction pairs from \airbnb.
\textbf{Losses} on second row:
M: masking;
P: pairing;
S: shuffling.
Row 1 corresponds to \vlnbert~\cite{majumdar2020vlnbert}.
% while the row 5 indicated through * employs the best path-instruction creation method.
}
\vspace{-2mm}
\label{tab:where}
\end{table}


% \begin{table*}[t]
% \centering
% \tabcolsep=0.1cm
% \begin{tabular}{@{\extracolsep{4pt}}r cccc ccccc ccccc @{}}
% \toprule
% \textbf{Step} & Replace CC & After CC & After CC & After R2R & \multicolumn{5}{c}{\textbf{Val Seen}} & \multicolumn{5}{c}{\textbf{Val Seen}} \\
% \cline{6-10} \cline{11-15}
% \textbf{Pair} & Image-capt. & Image-capt. & Path-instr. & Path-instr. & PL & NE & SPL & OSR & SR & PL & NE & SPL & OSR & SR \\
% \midrule
% % vanilla
% 1 &            &             &           &            
%     & 10.28 & 3.72 & 0.66 & 76.49 & \h 70.20
%     & 9.59 & 4.10 & 0.55 & 69.22 & \h 59.26 \\
% % Replace CC  bnbMN_r2rM_r2rR_scratch
% 2 & \checkmark &             &           &            &  \\
% % After CC imag-caption  bnbMN_r2rM_r2rR
% 3 &            & \checkmark  &           &            
%     & 10.14 & 3.62 & 0.69 & 78.0 & \h 72.13 
%     & 9.64 & 3.77 & 0.59 & 72.07 & \h 63.21 \\
% % After CC imag-caption  bnbMS_r2rM_r2rR
% 4 &            &             & \checkmark&            
%     & xx.xx & x.xx & x.xx & xx.x & \h xx.xx 
%     & x.xx & x.xx & x.xx & xx.xx & \h xx.xx \\
% % After R2R  r2rM_bnbMS_r2rR
% 5 &            &             &           & \checkmark 
%     & 10.32 & 3.53 & 0.70 & 79.04 & 73.84
%     & 9.85 & 3.92 & 0.58 & 72.71 & 62.71
% \\
% % After R2R  r2rM_bnbMS_r2rRS_indoor
% % 5 &            &             &           & \checkmark 
% %     & 9.52 & 3.44 & 0.69 & 77.47 & 71.69 
% %     & 9.36 & 3.85 & 0.59 & 70.03 & 63.47 \\

% % bnbMN_bnbMS_r2rM_r2rRS
% 6 &            & \checkmark  & \checkmark&            &  \\
% % bnbMN_r2rM_bnbMS_r2rRS
% 7 &            & \checkmark  &           & \checkmark &  \\
% \bottomrule
% \end{tabular}
% \caption{\vlnbert~\cite{majumdar2020vlnbert} pre-training consists in applying a masking/matching loss on an image-caption pair from Conceptual Captions~\cite{ConceptualCaptions} (CC), followed by a masking loss path-instruction pairs from VLN. The downstream task applies the ranking loss on VLN (no shuffling loss). This table compares the several options to apply Airbnb pre-training}
% \label{tab:where}
% \end{table*}
